Transformers as Support Vector Machines

Since its inception in "Attention Is All You Need", transformer architecture has led to revolutionary advancements in NLP. The attention layer within the transformer admits a sequence of input tokens $X$ and makes them interact through pairwise similarities computed as softmax$(XQK^\top X^\top)$, where $(K,Q)$ are the trainable key-query parameters. In this work, we establish a formal equivalence between the optimization geometry of self-attention and a hard-margin SVM problem that separates optimal input tokens from non-optimal tokens using linear constraints on the outer-products of token pairs. This formalism allows us to characterize the implicit bias of 1-layer transformers optimized with gradient descent: (1) Optimizing the attention layer with vanishing regularization, parameterized by $(K,Q)$, converges in direction to an SVM solution minimizing the nuclear norm of the combined parameter $W=KQ^\top$. Instead, directly parameterizing by $W$ minimizes a Frobenius norm objective. We characterize this convergence, highlighting that it can occur toward locally-optimal directions rather than global ones. (2) Complementing this, we prove the local/global directional convergence of gradient descent under suitable geometric conditions. Importantly, we show that over-parameterization catalyzes global convergence by ensuring the feasibility of the SVM problem and by guaranteeing a benign optimization landscape devoid of stationary points. (3) While our theory applies primarily to linear prediction heads, we propose a more general SVM equivalence that predicts the implicit bias with nonlinear heads. Our findings are applicable to arbitrary datasets and their validity is verified via experiments. We also introduce several open problems and research directions. We believe these findings inspire the interpretation of transformers as a hierarchy of SVMs that separates and selects optimal tokens.

==> sections/exp_report.tex <==
\section{Experiments}

\begin{figure}[t]
\centering
\hspace{-10pt}
\subfigure[Gradient path]{
    \includegraphics[width=.33\columnwidth]{figs/GD_path.pdf}
    \label{fig:path}
    
}%\caption{Global convergence}
\hspace{-10pt}
\subfigure[Correlations when training $\W$]{
    \includegraphics[width=.33\columnwidth]{figs/corr_W.pdf}
    \label{fig:corr W}
    
}%\caption{Convergence to global and local optima}
\hspace{-10pt}
\subfigure[Correlations when training $\Kb,\Qb$]{
    \includegraphics[width=.33\columnwidth]{figs/corr_KQ.pdf}
    \label{fig:corr KQ}
}
\vspace{-2mm}
\caption{The convergence behavior of the gradient descent on the attention weights $\W$ or $(\Kb,\Qb)$ using the logistic loss. 
% (a) Let $\W$ The arrows ({\color{gray} \footnotesize{--->---}}) represent trajectories from different initializations. Here, ({\color{red}-~-~-}) and ({\color{blue}-~-~-}) denote the \textbf{g}lobally- and \textbf{l}ocally-optimal \textbf{m}ax-\textbf{m}argin directions (\GM, \LM). $\gamma$ denotes the \emph{score} of a token per Definition \ref{score def}. 
}
\label{fig:main_fig}\vspace{-5pt}
\end{figure}
\begin{figure}[t]
\centering
\hspace{-10pt}
\subfigure[Gradient path]{
    \includegraphics[width=.33\columnwidth]{figs/GD_path_1.pdf}
    \label{fig:path 1}
    
}%\caption{Global convergence}
\hspace{-10pt}
\subfigure[Correlations when training $\W$]{
    \includegraphics[width=.33\columnwidth]{figs/corr_W_1.pdf}
    \label{fig:corr W 1}
    
}%\caption{Convergence to global and local optima}
\hspace{-10pt}
\subfigure[Correlations when training $\Kb,\Qb$]{
    \includegraphics[width=.33\columnwidth]{figs/corr_KQ_1.pdf}
    \label{fig:corr KQ 1}
}
\vspace{-2mm}

\hspace{-10pt}
\subfigure[Gradient path]{
    \includegraphics[width=.33\columnwidth]{figs/GD_path_0.pdf}
    \label{fig:path 0}
    
}%\caption{Global convergence}
\hspace{-10pt}
\subfigure[Correlations when training $\W$]{
    \includegraphics[width=.33\columnwidth]{figs/corr_W_0.pdf}
    \label{fig:corr W 0}
    
}%\caption{Convergence to global and local optima}
\hspace{-10pt}
\subfigure[Correlations when training $\Kb,\Qb$]{
    \includegraphics[width=.33\columnwidth]{figs/corr_KQ_0.pdf}
    \label{fig:corr KQ 0}
}
\vspace{-2mm}
\caption{Other results when using different $\z_i$s.
}
\label{fig:main_fig 01}\vspace{-5pt}
\end{figure}
\begin{itemize}
    \item Set $n=d=2$, $T=3$. $\x_{it}$ are randomly sampled from unit sphere, and $\vb=[0~1]^\top$ and labels $Y_i$ are all ones. 
    \item Figure~\ref{fig:main_fig} shows the convergence results when training with attention weights $\W$ or $(\Kb,\Qb)$. For simplicity, let $\tilde{\W}=\Qb\Kb^\top$. To visualize the gradient evolution, we focus on $\W\z_i$ and $\tilde\W\z_i$ for $i\in[n]$, so that it will clearly show how $\W\z_i$ ($\tilde\W\z_i$) converges in direction to the max-margin direction within each input. Fig.~\ref{fig:path}: Cyan and green markers represent different inputs and the stars are the optimal token within each input. Solid lines (red and blue) represent $\Ws_F\z_1$ and $\Ws_F\z_2$ and dashed lines represent $\Ws_\star\z_1$ and $\Ws_\star\z_2$ (we are overlaping). We also plot the trajectories $\W(t)\z_i$ and $\tilde\W(t)\z_i$, $i\in\{1,2\}$ in solid and dashed arrows. 
    \item Fig.~\ref{fig:corr W} and \ref{fig:corr KQ}: Define the correlation of two matrices $\W_1,\W_2\in\R^{d\times d}$ as follows: 
    \[
    \text{corr($\W_1,\W_2$)}=1-\left\|\frac{\W_1}{\|\W_1\|_F}-\frac{\W_2}{\|\W_2\|_F}\right\|_F^2.
    \]
    Then in Fig.~\ref{fig:corr W}, blue and orange curves show evolutions of corr($\W(t),\Ws_F$) and corr($\W(t),\Ws_\star$), respectively, and in Fig.~\ref{fig:corr KQ}, blue and orange curves represent corr($\tilde\W(t),\Ws_F$) and corr($\tilde\W(t),\Ws_\star$).
    \item \textbf{Random Data Experiments}: Set $n=T=3$ and $d=4$. $\x_{it}$ and $\vb$ are randomly sampled from unit sphere, and $Y_i$ are uniformly $\pm1$. Conduct $100$ random and successful trials ensuring that 1) attention succeeds in selecting one token per input, $\max_{t\in[T]}\sft{\X_i\W\z_i}_t=1$; 2) problems are separable and \eqref{eqn:sattnsvm} are feasible. Then over the $100$ trials, the averaged correlations are
    \[
    [\text{corr($\W,\Ws_F$)}~~\text{corr($\W,\Ws_\star$)}]=[0.997~~ 0.726],
    \]
    \[
    [\text{corr($\tilde\W,\Ws_F$)}~~\text{corr($\tilde\W,\Ws_\star$)}]=[0.749~~0.898].
    \]
    If setting $\tilde\W(0)=\Ws_\star$, then
    \[
    [\text{corr($\tilde\W,\Ws_F$)}~~\text{corr($\tilde\W,\Ws_\star$)}]=[0.769~~0.982].
    \]
    \item \textbf{Random Data Experiments v2}: Set $n=4,T=4,d=20$ and train with cross attention where $\z_{i}$'s are also randomly sampled from unit sphere. Results averaged form $100$ trials are
    \[
    \text{Frob:}~[\text{corr($\tilde\W,\Ws_F$)}~~\text{corr($\tilde\W,\Ws_\star$)}]=[0.996~~0.607].
    \]
    \[
    \text{Nuc:}~~[\text{corr($\tilde\W,\Ws_F$)}~~\text{corr($\tilde\W,\Ws_\star$)}]=[0.692~~0.840].
    \]
    \begin{enumerate}
        \item After setting $\Kb,\Qb\in\R^{d\times m}$ to be low rank with  $m=rank(\Wso)$, we obtain
        \[
    \text{Nuc:}~~[\text{corr($\tilde\W,\Ws_F$)}~~\text{corr($\tilde\W,\Ws_\star$)}]=[0.695~~0.837].
    \]
    \item After setting $\Kb(0)=\Ub\bSi^{1/2}+0.1\cdot\Nc(0,\Iden)$ and $\Qb(0)=\Vb\bSi^{1/2}+0.1\cdot\Nc(0,\Iden)$ where $\Ub\bSi\Vb=\Wso/\|\Wso\|$, we obtain
    \[
    \text{Nuc:}~~[\text{corr($\tilde\W,\Ws_F$)}~~\text{corr($\tilde\W,\Ws_\star$)}]=[0.634~~0.968].
    \]
    \item Combining low rank and initialization together, we obtain
    \[
    \text{Nuc:}~~[\text{corr($\tilde\W,\Ws_F$)}~~\text{corr($\tilde\W,\Ws_\star$)}]=[0.598~~0.979].
    \]
    \end{enumerate}

\end{itemize}

\begin{figure}[t]
\centering
\hspace{-10pt}
    \includegraphics[width=.5\columnwidth]{figs/diff_nT.pdf}
    \label{fig:diff nT}
    

\caption{The probabilities of global convergence. We train attention weight $\W$ with different $(n,T,d)$ choices, and examine the probabilities of global convergence under each setting. Here, $\W$ globally converges in direction to $\Wso$ only if $\arg\max_{t\in[T]}\sft{\X_i\W\z_{i}}_t=\op_i$ for all $i\in[n]$.
}
\label{fig:main_fig}\vspace{-5pt}
\end{figure}

==> sections/experiments.tex <==
\section{Experiments}\label{sec:exprim}


\red{
TODO:
\begin{itemize}
    \item \textbf{Page 2}: visualization using $\W\z$ + overparam + ?
    \item Low rank experiment: vary $m$ and train $(\Kb,\Qb)$
    \item Nonlinear head e.g. ReLU function
    \item Self attention using $\V$
\end{itemize}
}

\red{[Move this part to Experiment section?]}\ct{agree}

 
%, Above, we assumed that $(\Kb,\Qb)$-parameterization is full dimensional i.e. $m=d$. Intuitively, setting $m<d$ should promote a low-rank bias (beyond nuclear norm) as $\Kb\Qb^\top$ is at most rank $m$ by construction.
%unconstrained solutions are .  

%Also remark that we can capture local geometry as discussed in Sec 3.\\(2) Add and discuss experiments on Frobenius and Nuclear norm supporting the conclusions.\\(3) Ideally, we should have an experiment with $m<d$ and another with $h(x)=\onebb^\top\texttt{ReLU}(\Vb\x)$. The former is easy! Whenever sample size is $n\leq d$, you automatically have rank-$n$ solution.}

==> sections/fig_nn_corrs.tex <==
\begin{figure}
    \centering
    \hspace{-10pt}
    \subfigure[$\W^{\text{adapt}}$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[height=.22\columnwidth, trim={1.3cm 1.3cm 0 0}, clip]{figs/nn_corr_itr_adapt.pdf}};
        \node at (0,-2.) {\small{Iterations}};
        \node[rotate=90] at (-2.65,0) {\small{$1-$correlation coefficient}};
        \end{tikzpicture}
        \label{fig nn corr adapt}
    }
    \hspace{-10pt}
    \subfigure[$\Ws$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[height=.22\columnwidth, trim={1.3cm 1.3cm 0 0}, clip]{figs/nn_corr_itr_svm.pdf}};
        % \node[rotate=90] at (-2.7,0) {\small{$1-$correlation coefficient}};
        \node at (0,-2.){\small{Iterations}};
        \end{tikzpicture}
        \label{fig nn corr svm}
    }
    \hspace{-10pt}
    \subfigure[$\W^\dagger$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[height=.22\columnwidth, trim={1.3cm 1.3cm 0 0}, clip]{figs/nn_corr_itr_single.pdf}};
        \node at (0,-2.) {\small{Iterations}};
        % \node[rotate=90] at (-2.65,0) {\small{$1-$correlation coefficient}};
        \end{tikzpicture}
        \label{fig nn corr single}
    }
    \caption{} 
    \label{fig nn corrs}
\end{figure}

==> sections/fig_overparam_app.tex <==
\begin{figure}[t]
    \centering
    % \subfigure[$\W$-parameterization]{
    %     \begin{tikzpicture}
    %     \node at (0,0) {\includegraphics[height=.22\columnwidth, trim={1.3cm 1.3cm 3.2cm 0}, clip]{figs/overparam_W_bar.pdf}};
    %     \node[rotate=90] at (-4,0) {\small{Probabilities}};
    %     \node at (-1,-2.){\small{$d$}};
    %     \node at (2.9,1.4){\small{Not-local}};
    %     \node at (2.9,1.1){\small{Global}};
    %     \node at (2.9,0.75){\small{Local}};
    %     \node at (2.9,0.4){\small{Asmp B.1}};
    %     \end{tikzpicture}
    %     \label{fig overparam W bar2}
    % }
    \subfigure[Train attention weights $\Kb,\Qb\in\R^{d\times m}$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[height=.25\columnwidth, trim={1.2cm 1.4cm 0 0}, clip]{figs/rank_diff_m.pdf}};
        \node at (0,-2.2) {\small{{Varying $m$}}};
        \node[rotate=90] at (-3.1,0) {\small{$1-$correlation coefficient}};
        \end{tikzpicture}
        \label{fig rank m}
    }
    \hspace{10pt}
    \subfigure[Convergence types of $(\Kb,\Qb)$-parameterization]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[height=.25\columnwidth, trim={1.3cm 1.2cm 3.2cm 0}, clip]{figs/overparam_KQ_bar.pdf}};
        \node[rotate=90] at (-4.3,0) {\small{Percentage}};
        \node at (-1,-2.2){\small{Varying $d$}};
        \node at (3.2,1.6){\small{Not Local}};
        \node at (3.2,1.24){\small{Global}};
        \node at (3.2,0.87){\small{Local}};
        \node at (3.2,0.5){\small{Assum B.1}};
        \end{tikzpicture}
        \label{fig overparam KQ bar}
    }
    \caption{ Convergence behavior of GD when training cross-attention weights $\W$ (solid) or $(\Kb,\Qb)$ (dashed) with random data and varying $m$ and $d$. \textbf{(a)}: Fixing dimensionality at $d=20$, attention weights $\Kb,\Qb\in\R^{d\times m}$ are trained for $m\leq10$. The misalignment between attention SVM and GD, $1-\corr{\Ws_{\star,\bal},\Kb\Qb^\top}$, is studied. $\Ws_{\star,\bal}$ is from \eqref{eqn:sattnsvmst} with GD tokens $\bal$ and $m=d$. Subfigures with fixed $n=5$ and $T=5$ show that as $m$ approaches or exceeds $n$, $\Kb\Qb^\top$ aligns more with $\Ws_{\star,\bal}$.  \textbf{(b)}: Red, blue, and teal bars represent the percentages of Global, Local (including Global), and Not Local convergence, respectively. The green bar corresponds to Assumption \ref{assum:token:supp} where all tokens act as support vectors. Larger overparameterization ($d$) relates to a higher percentage of optimal SVM convergence.} 
    \label{fig overparam bar}
\end{figure}

==> sections/zzz_prelim.tex <==
\begin{comment}
Let us now shift our focus towards solving the SVM problem using optimal indices denoted by $(\opt_i)_{i=1}^n$. It is important to note that the problem can be formulated for arbitrary sets of indices $\boldsymbol{\alpha} = (\alpha_i)_{i=1}^n$, which will reveal locally optimal directions, as defined in Section~\ref{sec local}. We introduce the following formulation:
\begin{tcolorbox}[colback=white!5!white,colframe=black!5!black,colback=green!1!white]
\begin{equation}\tag{\name}
\Wm_\dm=\arg\min_{\W}\td{\W}
\quad \text{subject to} \quad \min_{t\neq \op_i}(\x_{i\op_i}-\x_\itt)^\top\W\z_i\geq 1\quad \text{for all} \quad 1\leq i\leq n\label{eqn:sattnsvm}.
\end{equation}
\end{tcolorbox}
In \eqref{eqn:sattnsvm}, we use $\diamond$ to denote a generic objective function that captures the inductive bias of the optimization problem. Throughout our discussion, we will use $\Wm$ to represent the unique solution of \eqref{eqn:sattnsvm} with the Frobenius norm objective, and $\Wm_\star$ to denote the solution of \eqref{eqn:sattnsvm} with the nuclear norm. In the following, we provide insights and discussions on the implicit bias of gradient descent applied to \eqref{eqn:erm:w} towards $\Wm$. In the next section, we delve into discussions on $\Wm_\star$ and its connection to \eqref{eqn:erm:kq} and the SVM problem parameterized by $(\Kb,\Qb)$.
%, which represents the unique solution of \eqref{eqn:sattnsvm} with the Frobenius norm.
%As we shall see, $\Wm$ corresponds to the implicit bias of gradient descent applied to the \eqref{eqn:erm:w} formulation parameterized by $\W$. 


It is worth noting that the existence of matrix $\Wm$ implies the separability of tokens $\op_i$ from the others. Additionally, the term $a_{\itt}=\x_\itt^\top\W\z_i$ represents the dot product between the key-query features before applying the softmax nonlinearity. This dot product is a crucial characteristic of self-attention. Therefore, we can express the SVM constraints in \eqref{eqn:sattnsvm} as $a_{i\op_i}\geq a_{\itt}+1$. This formulation aims to find the most efficient direction that ensures the optimal token $\x_{i\op_i}$ achieves the highest similarity with query $\z_i$ among all key embeddings.

To gain further insight into equation \eqref{eqn:sattnsvm}, let's consider that the output token of the attention layer is a convex mixture of the input tokens. If the training loss is minimized by selecting the optimal token $\x_{i\op_i}$, then the softmax similarities should converge to a one-hot vector that precisely includes $\x_{i\op_i}$ (assigned a value of 1) and disregards all other tokens (assigned 0s). For this convergence to occur, the attention weights $\W$ should diverge in norm to saturate the softmax probabilities. However, the weights converge in direction to the max-margin SVM due to the exponential-tailed nature of the softmax function. This phenomenon resembles the inductive bias of logistic regression on separable data \cite{soudry2018implicit,ji2018risk}. Lemma \ref{lem min risk} formalizes this intuition and provides a rigorous motivation for our definition of optimal tokens.


% We now turn our attention to solving the SVM problem using optimal indices denoted by $ (\opt_i)_{i=1}^n$. It is important to note, however, that the problem can be formulated for arbitrary sets of indices $\boldsymbol{\alpha} = (\alpha_i)_{i=1}^n$, which will reveal locally-optimal directions; see Definition~\ref{sec local}.
% %
% \tcbset{colback=white!5!white,colframe=black!5!black,colback=green!1!white}
% \begin{tcolorbox}%[height=1cm, width=15cm]
% \begin{equation}\tag{\name}
% \Wm_\dm=\arg\min_{\W}\td{\W}
%  \quad \text{subj. to}   \quad \min_{t\neq \op_i}(\x_{i\op_i}-\x_\itt)^\top\W\z_i\geq 1\quad \text{for all} \quad 1\leq i\leq n\label{eqn:sattnsvm}.
% \end{equation}
% \end{tcolorbox}
% Here, we use $\diamond$ to denote a generic objective function capturing the inductive bias of the optimization problem. Thourghout, we will use to denote $\Wm$ be the unique solution of \eqref{eqn:sattnsvm} with Frobenius norm, and $\Wc^\svm_\star$ be the solution set of \eqref{eqn:sattnsvm} with nuclear norm and cost function $\tnuc{\Wc^\svm_\star}$. 



% We first provide insights and discussions on the implicit bias of gradient descent applied to \eqref{eqn:erm:w} towrads  $\Wm$ as be the unique solution of \eqref{eqn:sattnsvm} with Frobenius norm. As we shall see,  $\Wm$ will correspond to implicit bias of gradient descent applied to the \eqref{eqn:erm:w} parameterized by $\W$. In the next section, we provide discussions on $\Wm_c$ and how it is connected to   \eqref{eqn:erm:kq} and $(\Kb,\Qb)$ parameterized SVM problem.



% Note that the existence of matrix $\Wm$ implies the separability of tokens $\op_i$ from the others. Additionally, the term $a_{\itt}=\x_\itt^\top\W\z_i$ represents the dot product between the key-query features before applying the softmax nonlinearity. This dot product is a crucial characteristic of self-attention. Therefore, we can express the SVM constraints in \eqref{eqn:sattnsvm} as $a_{i\op_i}\geq a_{\itt}+1$. This formulation aims to find the most efficient direction that ensures the optimal token $\x_{i\op_i}$ achieves the highest similarity with query $\z_i$ among all key embeddings.  To gain further insight into equation \eqref{eqn:sattnsvm}, let's consider that the output token of the attention layer is a convex mixture of the input tokens. If the training loss is minimized by selecting the optimal token $\x_{i\op_i}$, then the softmax similarities should converge to a one-hot vector that precisely includes $\x_{i\op_i}$ (assigning a value of 1) and disregards all other tokens (assigning 0s). In order for this convergence to happen, the attention weights $\W$ should diverge in norm to saturate the softmax probabilities. However, the weights converge in direction to the max-margin SVM due to the exponential-tailed nature of the softmax function. This phenomenon is similar to the inductive bias of logistic regression on separable data \cite{soudry2018implicit,ji2018risk}. Lemma \ref{lem min risk} formalizes this intuition and provides rigorous motivation for our optimal token definition.

% Note that the existence of $\Wm$ implies the separability of tokens $\op_i$ from the others. Furthermore, $a_{\itt}=\x_\itt^\top\W\z_i$ represents the dot product between the key-query features before the softmax nonlinearity, which is an essential feature of self-attention. Therefore, the SVM constraints in \eqref{eqn:sattnsvm} can be expressed as $a_{i\op_i}\geq a_{\itt}+1$. This formulation can be interpreted as seeking the most efficient direction that ensures the optimal token $\x_{i\op_i}$ achieves the highest similarity with query $\z_i$ among all key embeddings.  To provide further insight into \eqref{eqn:sattnsvm}, consider that the output token of the attention layer is a convex mixture of the input tokens. If the training loss is minimized by selecting the optimal token $\x_{i\op_i}$, then the softmax similarities should converge to a one-hot vector that precisely includes $\x_{i\op_i}$  (assigning a value of 1) and disregards all other tokens (assigning 0s). For this to occur, the attention weights $\W$ should diverge in norm to saturate the softmax probabilities. However, the weights converge in direction to the max-margin SVM due to the exponential-tailed nature of the softmax function. This phenomenon is similar to the inductive bias of logistic regression on separable data \cite{soudry2018implicit,ji2018risk}. This intuition is formalized in Lemma \ref{lem min risk} which also rigorously motivates our optimal token definition.




%\smallskip

% Above $\diamond$ denotes a generic objective function capturing the inductive bias of the optimization problem: As we shall see, it will correspond to the Frobenius norm when the problem is parameterized by $\W$. On the other hand, $(\Kb,\Qb)$ parameterization with $\W\gets\Kb\Qb^\top$ will be biased towards minimizing nuclear norm. 

\subsection{Non-convex hard-margin SVM problem for cross attention with parameters $(\mathbf{Q},\mathbf{K})$ } 

The objective function in \eqref{eqn:erm:kq} generally lacks convexity in terms of $(\Qb, \Kb)$. However, when training without regularization \footnote{ maybe give $\lambda=1e-16$...} the token separation with a maximum margin occurs. In this case, gradient descent update \ref{GD-QK}  produces iterations that diverge in norm but converge in direction (refer to Figure~\ref{fig path}). This behavior resembles the margin maximization observed in non-convex problems such as homogeneous neural networks \cite{lyu2019gradient,ji2020directional}, which is an implicit regularization effect of gradient descent. Notably, \cite{lyu2019gradient,ji2020directional} has demonstrated that solutions obtained through gradient descent and gradient flow converge in direction towards a Karush–Kuhn–Tucker (KKT) point of the max-margin SVM. Motivated by the aforementioned works and supported by preliminary experiments illustrated in Figure~\ref{fig path}, along with a comprehensive numerical study detailed in Section~\ref{sec:exprim}, we introduce a nonconvex SVM problem. This problem is parameterized by $(\Qb, \Kb)$ similar to its twin problem \eqref{eqn:erm:kq},  and its objective is to achieve a separation between the optimal tokens indexed by $(\opt_i)_{i=1}^n$ and
from the remaining tokens in the input sequence $\{\X_i\}_{i=1}^n$.
% Motivated by these works, and supported by initial experiments depicted in Figure~\ref{fig path} as well as a more extensive numerical study discussed in Section~\ref{sec:exprim}, we propose a nonconvex SVM problem 
% paramterized by $(\Qb, \Kb)$ that aims to separate  
% optimal tokens indexed by $(\opt_i)_{i=1}^n$ and
% from the remaining tokens in the input sequence $\{\X_i\}_{i=1}^n$.
\tcbset{colback=white!5!white,colframe=black!5!black,colback=green!1!white}
\begin{tcolorbox}[height=2cm]
\begin{equation}\tag{KQ-SVM}
\Kb,\Qb=\arg\min_{\Kb,\Qb}~\frac{1}{2} \left(\|\Kb\|_F^2+\|\Qb\|_F^2\right)
 \quad \text{subj. to}   \quad \min_{t\neq \op_i}(\x_{i\op_i}-\x_\itt)^\top\Kb\Qb^\top\z_i\geq 1\quad \text{for all} \quad 1\leq i\leq n\label{eqn:qk:svm}.
\end{equation}
\end{tcolorbox}
%
% A KKT point satisfies certain conditions, known as KKT conditions, which were proven to be necessary for optimality of certen problems that in the case
% of homogeneous neural networks, these
% conditions are necessary for optimality. However, they are not sufficient
% even for local optimality 
% . However, these conditions are not sufficient for local optimality. Therefore,

A KKT point does not always represent an optimal solution for the maximum-margin problem. This is analogous to showing that an unconstrained optimization problem reaches a point where the gradient is zero, without proving whether it is a global minimum, local minimum, or saddle point. While convergence to a KKT point in the \eqref{eqn:qk:svm} formulation indicates a tendency towards maximizing the margin in the parameter space, it does not provide a guarantee for reaching a maximum-margin solution.

Our objective is to demonstrate that the non-convex optimization problem \eqref{eqn:erm:kq} at hand is not as daunting as it may initially seem. Specifically, we aim to establish that, apart from the global optimum, all other KKT points  act as saddle points that can be circumvented through gradient descent updates \ref{GD-QK}. In fact, we identify the implicit regularizer as the \textit{nuclear norm} and illustrate that, even in the absence of constraints on the factored matrix $\W=\Kb\Qb^\top$ and employing a full-dimensional factorization, optimization through gradient descent on the $(\Qb, \Kb)$ factorization directs us towards the solution of \eqref{eqn:sattnsvm} with the minimum nuclear norm, i.e. $\Wm_\star$.   Our empirical investigation allows us to conjecture that, with appropriate step size,  \ref{GD-QK} converges to the solution of \eqref{eqn:sattnsvm} with the minimum nuclear norm, and we provide empirical evidence to support this conjecture, substantiating it within certain restricted settings.
\end{comment}

% To provide further intuition on \eqref{eqn:sattnsvm}, note that, the output token of the attention layer is a convex mixture of input tokens. If the training loss is minimized by selecting the optimal token $\x_{i\op_i}$, then, softmax similarities should converge to a one-hot vector that precisely includes $\x_{i\op_i}$ (by assigning 1) and discards all other tokens (by assigning 0s). For this to happen, the attention weights $\W$ should diverge in norm to saturate the softmax probabilities. However, the weights converge in direction to the max-margin SVM thanks to the fact that softmax function is exponentially-tailed. This phenomenon is akin to the inductive bias of logistic regression on separable data \red{\cite{}}.
%Thus, the SVM constraints of \eqref{eqn:sattnsvm} are of the form $a_{i\op_i}\geq a_\itt+1$. This has the following interpretation: \eqref{eqn:sattnsvm} is seeking for the most efficient direction that ensures optimal token $\x_{i\op_i}$ achieves largest similarity with query $\z_i$ among all key embeddings.
%The high-level intuition underlying \eqref{eqn:sattnsvm} is as follows: 
%what remains unknown is the specific performance metric $\W$ will optimize. To capture this uncertainty, we introduce a generic norm denoted by $\diamond$. Several potential candidates for the $\diamond$ norm include the Frobenius norm $\|\cdot\|_F$, the Nuclear norm $\|\cdot\|_\star$, the Spectral norm $\|\cdot\|$, and the $\ell_2$ margin minimizer $\|\W\|_{\diamond}=\min_{i\in[n]} \tn{\W\z_i}$. This leads us to our conjecture.
%of the attention has to be saturated to guarantee  If the training loss benefits from atte
%Given the exponentially-decaying tail of the softmax function, we expect attention mechanism to exhibit a bias towards selecting the optimal token that minimizes the empirical risk, assuming the tokens are separable. However, what remains unknown is the specific performance metric $\W$ will optimize. To capture this uncertainty, we introduce a generic norm denoted by $\diamond$. Several potential candidates for the $\diamond$ norm include the Frobenius norm $\|\cdot\|_F$, the Nuclear norm $\|\cdot\|_\star$, the Spectral norm $\|\cdot\|$, and the $\ell_2$ margin minimizer $\|\W\|_{\diamond}=\min_{i\in[n]} \tn{\W\z_i}$. This leads us to our conjecture.
